An Efficient Evolutionary Algorithm for Diversified Top-k (Weight) Clique Search Problems

In many real-world problems and applications, finding only a single element, even though the best, among all possible candidates, cannot fully meet the requirements. We may wish to have a collection where each individual is not only outstanding but also distinctive. Diversified Top-k (DTk) problems are a kind of combinatorial optimization problem for finding such a promising collection of multiple sub-structures, such as subgraphs like cliques and social communities. In this paper, we address two representative and practical DTk problems, DTk Clique search (DTkC) and DTk Weight Clique search (DTkWC), and propose an efficient algorithm called Diversified Top-k Evolutionary AlgorithM (DiverTEAM) for these two problems. DiverTEAM consists of a local search algorithm, which focuses on generating high-quality and diverse individuals and sub-structures, and a genetic algorithm that makes individuals work as a team and converge to (near-)optima efficiently. Extensive experiments show that DiverTEAM exhibits an excellent and robust performance across various benchmarks of DTkC and DTkWC.

==> body/04-Framework.tex <==
This section introduces our DiverTEAM evolutionary algorithm proposed for DT$k$C and DT$k$WC.

%, based on the definitions introduced in Section~\ref{sec-Pre}. Note that due to the similarity between DT$k$ problems, those definitions can be easily adjusted to define other DT$k$ problems. For instance, when solving the DT$k$ biclique search problem~\cite{LQL+22} and DT$k$ community search problem~\cite{SWW+22}, we may directly regard the symbol $c$ as a biclique or social community, and $C$ as a combination of bicliques or social communities. The optimization objective $W(C)$ and definitions $priv(c, C)$ and $score(c, C)$ can then be adjusted accordingly to fit these DT$k$ problems. Then, DiverTEAM can also be directly applied to these problems.

%DiverTEAM consists of local search and genetic algorithms. %In DiverTEAM, a solution $C$ is regarded as an individual in the population, and a sub-structure $c$ is regarded as a gene. %The search operator used to improve an individual in local search and genetic algorithms is also unified, \ie, single gene substitution that substitutes one of the genes in the individual with a new one.
%Both the local search and genetic algorithms in DiverTEAM improve an individual by replacing one of its genes with a new one. 
In the following, we first introduce the main process of DiverTEAM, and then present its two procedures, the local search and genetic algorithms. %, respectively.


\subsection{Main Process of DiverTEAM}
The main procedure of DiverTEAM is shown in Algorithm~\ref{alg_DiverTEAM}. DiverTEAM separates the local search and genetic algorithms into two stages. In the first stage (lines 3-6), a local search algorithm, \ie, function LocalSearch(), is used to generate individuals in the population. In the second stage (lines 7-10), a genetic algorithm, \ie, function GeneticAlg() is used to search with the population. The two stages have their own stopping conditions (\textit{\uppercase\expandafter{\romannumeral1}} and \textit{\uppercase\expandafter{\romannumeral2}}), which can be adjusted to fit different limitations for the algorithm, \eg, limits of calculation time or memory. The stopping conditions in our implementation of DiverTEAM for DT$k$WC and DT$k$C are referred to in Section~\ref{sec-Details}.

%Usually, the calculation time of the algorithm is limited by a cut-off time $T$. 

\iffalse
\begin{algorithm}[t]
\caption{The main process of DiverTEAM}
\label{alg_DiverTEAM}
\LinesNumbered 
\KwIn{A DT$k$ instance $G$, an integer $k$, the maximum unimproved step in local search $M_{step}$}
\KwOut{A solution $C$ of $G$}
$IV \leftarrow$ set of isolated vertices with degree 1\;
$LV \leftarrow$ set of leaf vertices with degree 0\;
Initialize the population $P \leftarrow \emptyset$\;
Initialize the best solution $C^* \leftarrow \emptyset$\;
\While{stopping condition \uppercase\expandafter{\romannumeral1} is not met}{
$C \leftarrow$ LocalSearch($G$, $k$, $M_{step}$, $IV$, $LV$)\;
$C \leftarrow$ FixReduction($G$, $C$, $IV$, $LV$)\;
\lIf{$W(C) > W(C^*)$}{$C^* \leftarrow C$}
$P \leftarrow P \cup \{C\}$\;
}
\While{stopping condition \uppercase\expandafter{\romannumeral2} is not met}{
$P \leftarrow$ GeneticAlg($G$, $P$, $k$)\;
$C_{max} \leftarrow \arg\max_{C \in P}{W(C)}$\;
\lIf{$W(C_{max}) > W(C^*)$}{$C^* \leftarrow C_{max}$}
}
$P \leftarrow$ PostPrecess()\;
\textbf{return} $C^*$\;
\end{algorithm}
\fi



\begin{algorithm}[t]
\fontsize{10.1pt}{15}
\caption{The main process of DiverTEAM}
\label{alg_DiverTEAM}
\LinesNumbered 
\KwIn{A graph $G$, an integer $k$, the maximum unimproved step in local search $M_{step}$}
\KwOut{A solution $C$}
Initialize the population $P \leftarrow \emptyset$\;
Initialize the best solution $C^* \leftarrow \emptyset$\;
\While{stopping condition \uppercase\expandafter{\romannumeral1} is not met}{
$C \leftarrow$ LocalSearch($G$, $k$, $M_{step}$)\;
%$C \leftarrow$ PostRedution$(G,C)$\;
\lIf{$W(C) > W(C^*)$}{$C^* \leftarrow C$}
$P \leftarrow P \cup \{C\}$\;
}
\While{stopping condition \uppercase\expandafter{\romannumeral2} is not met}{
$P \leftarrow$ GeneticAlg($G$, $P$, $k$)\;
$C_{max} \leftarrow \arg\max_{C \in P}{W(C)}$\;
\lIf{$W(C_{max}) > W(C^*)$}{$C^* \leftarrow C_{max}$}
}
%\For{\rm{\textbf{each} individual $C \in P$}}{$C \leftarrow$ postprocessing$(G,C)$\;
%\lIf{$W(C) > W(C^*)$}{$C^* \leftarrow C_{max}$}
%}
\textbf{return} $C^*$\;
\end{algorithm}



\subsection{Local Search Process}
The procedure of the local search algorithm in DiverTEAM is presented in Algorithm~\ref{alg_LocalSearch}. The algorithm first constructs a solution $C$ by merging $k$ genes (lines 1-3). Each gene is found by function FindGene() (line 3), which can be designed flexibly for different DT$k$ problems. Then, the algorithm 
iteratively adds a gene found by FindGene() into $C$ and removes the gene with the minimum $score$ from $C$ until %the stopping condition \textit{\uppercase\expandafter{\romannumeral1}} (\eg, cut-off time) is met (line 5) or \
the maximum unimproved step $M_{step}$ is reached (line 5).


Note that during the local search process, solution $C$ never becomes worse because the added and removed genes can be the same. Since DT$k$ problems usually have huge solution spaces, different from HEA-D using simulated annealing methods to accept worse solutions, we prohibit the solution from getting worse during the local search, which can prevent the algorithm from being hard to converge. Since the genetic algorithm in DiverTEAM is very efficient, most of the running time (usually more than 3/4 of the total running time) is spent on local search in DiverTEAM, making the local search process concentrate on generating high-quality and diverse local optimal solutions for the population. 


%Moreover, in our DiverTEAM framework, the maximum unimproved step in local search, \ie, $M_{step}$, can be updated adaptively to fit different DT$k$ instances. For different instances, the hardness of escaping from local optima is distinct. Updating $M_{step}$ can help the algorithm select appropriate parameters adaptively for different instances. In our implementation, we empirically update $M_{step}$ to the number of steps of the last local search process divided by 4 (line 12). With the benefit of the above advantages, the local search process can generate high-quality local optimal solutions efficiently.


\begin{algorithm}[t]
\fontsize{10.1pt}{15}
\caption{LocalSearch($G$, $k$, $M_{step}$)}
\label{alg_LocalSearch}
\LinesNumbered 
\KwIn{A graph $G$, an integer $k$, the maximum unimproved step in local search $M_{step}$}
\KwOut{A solution $C$}
Initialize $C \leftarrow \emptyset$\;
\For{$i \leftarrow 1 : k$}{
$c \leftarrow$ FindGene($G$), $C \leftarrow C \cup \{c\}$\;
}
%Initialize $step \leftarrow 0$, $M_{step}' \leftarrow M_{step}$\;
Initialize $step \leftarrow 0$\;
%\While{stopping condition \uppercase\expandafter{\romannumeral1} is not met}{
\While{$step < M_{step}$}{
$step \leftarrow step + 1$\;
%\lIf{stopping condition \uppercase\expandafter{\romannumeral1} is met}{\textbf{break}}
$c \leftarrow$ FindGene($G$), $C' \leftarrow C \cup \{c\}$\;
$c_{min} \leftarrow \arg\min_{c \in C'}{score(c, C')}$\;
$C' \leftarrow C' \backslash c_{min}$\;
\If{$W(C') > W(C)$}{$C \leftarrow C'$, $step \leftarrow 0$\;}

%\lIf{$step \geq M_{step}$}{\textbf{break}}
}
%$M_{step} \leftarrow step/4$\;
\textbf{return} $C$\;
%\textbf{return} $\{C, M_{step}\}$\;
\end{algorithm}


\subsection{Genetic Algorithm}

The procedure of the genetic algorithm in DiverTEAM is presented in Algorithm~\ref{alg_GeneticAlg}.
At each generation, each individual is selected once as parent $C_1$ and once as parent $C_2$ in random order (lines 1-4). For each pair of parents, the algorithm tries to replace a gene $c_1 \in C_1$ with a gene $c_2 \in C_2$ to evolve $C_1$, and it traverses all possible replacements to find the best one (lines 5-11).

%The algorithm begins by randomly shuffling the input population $P$(line 1) and connecting the first individual to the end of $P$, thereby forming a directed ring. Afterwards, for each pair of connected individuals $C_1$ and $C_2$, we make an attempt to remove a gene from $C_1$ and select a gene from $C_2$ to incorporate into $C_1$. We iterate through all possible attempts and select the optimal action for modifying $C_1$ (lines 2-11).

Note that we have found sufficient high-quality and diverse genes through the local search process, which are distributed among various individuals in the population.
The goal of the genetic algorithm is to effectively propagate these promising genes throughout the entire population, enabling each individual to efficiently discover suitable genes that match their characteristics.
Importantly, the time complexity of function GeneticAlg() is $O(|P|k^2)$, allowing us to efficiently propagate the genes and evolve the population. Experimental results also demonstrate the superiority of our proposed genetic algorithm over that in HEA-D.


%throughout the population, % in a relatively short timeframe
%thereby accomplishing the aim of population evolution.





\begin{algorithm}[t]
\fontsize{10.1pt}{15}
\caption{GeneticAlg($G$, $P$, $k$)}
\label{alg_GeneticAlg}
\LinesNumbered 
\KwIn{A graph $G$, a population $P$, an integer $k$}
\KwOut{A population $P$}

Randomly shuffle $P$\;

%$C \leftarrow 1$-st individual in $P$\;

%$P \leftarrow$ push back $C$ to $P$\;

\For{$i \leftarrow 1 : |P|$}{

$C_1 \leftarrow i$-th individual in $P$\;

$C_2 \leftarrow (i \mod |P|+1)$-th individual in $P$\;

Initialize $score^* \leftarrow -\infty$, $c_1^* \leftarrow \emptyset$, $c_2^* \leftarrow \emptyset$\;

\For{\rm{\textbf{each}} gene $c_1 \in C_1$}{
\For{\rm{\textbf{each}} gene $c_2 \in C_2$}{

$score \leftarrow W(C_1\backslash \{c_1\} \cup \{c_2\}) - W(C_1)$\;

\If{$score > score^*$}{
    $score^* \leftarrow score$, $c_1^* \leftarrow c_1$, $c_2^* \leftarrow c_2$\;
}
}
}

$C_1 \leftarrow C_1\backslash \{c_1^*\} \cup \{c_2^*\}$\;

}

%$M_{step} \leftarrow step/4$\;
\textbf{return} $P$\;
%\textbf{return} $\{C, M_{step}\}$\;
\end{algorithm}

%\subsection{Deployment to Different Problems}
%\HK{Add a discussion on the general idea of how to deploy the framework to differenct DT$k$ problems. For DT$k$WC and DT$k$C,... For another one or two problems, ... }

==> body/05-Details.tex <==
In this section, we first introduce some techniques for improving the algorithm's performance and efficiency, including a pseudo graph reduction preprocessing, the solution-based tabu search method in the genetic algorithm, and several postprocessing methods. Actually, these methods are also not specific to these two problems but can be generalized to solve other DT$k$ problems. Then, we introduce some detailed implementations of DiverTEAM for the DT$k$WC and DT$k$C problems, including the stopping conditions \textit{\uppercase\expandafter{\romannumeral1}} and \textit{\uppercase\expandafter{\romannumeral2}}, and the FindGene() function used to find a gene (\ie, clique in DT$k$WC and DT$k$C) during the local search process.

%These methods also suggest an effective way to use the DiverTEAM framework to solve specific DT$k$ problems.
%the FindGene() function used to find a gene (\ie, clique in DT$k$C and DT$k$WC) during the local search process,



\subsection{Pseudo Graph Reduction Preprocessing}
In many real-world applications, such as social networks, graphs are massive and sparse. Thus, searching the entire graph is inefficient, and many graph reduction methods have been proposed for various problems over graphs~\cite{ZHX+21,XLY22}. Due to the complexity of DT$k$WC and DT$k$C, it is very hard to reduce the graph with theoretical guarantees. Inspired by the leaf vertex union match method~\cite{Zhou0ZL022} that ignores leaf vertices (with degree 1) and handles them when encountering their parent vertices, we propose a pseudo graph reduction method that ignores isolated vertices (with degree 0) and leaf vertices during the local search process and considers them after the process, so as to improve the search efficiency.


We denote the set of all isolated vertices as $IV$ and the set of all leaf vertices as $LV$. During the FindGene() function, vertices in $IV$ and $LV$ are not considered. Once the LocalSearch() function returns a solution $C$ (line 4 in Algorithm~\ref{alg_DiverTEAM}), we utilize a PostReduction() function to enhance the quality of $C$ by taking into account the ignored vertices. This function is depicted in Algorithm~\ref{alg_PostReduction}. It iterates through each isolated or leaf vertex and identifies the 
%clique $c'$ corresponding to them with size 2 or 1 (lines 3-4), 
corresponding clique $c'$ with size 2 or 1 (lines 3-4), 
trying to replace one of the cliques in $C$ with $c'$ for improvement 
(lines 5-8).


\iffalse
\begin{algorithm}[t]
\caption{FindGene($G$)}
\label{alg_FindGene}
\LinesNumbered 
\KwIn{A graph $G = (V, E)$}
\KwOut{A clique $c$}
$IV \leftarrow$ set of isolated vertices in $G$ with degree 0\;
$LV \leftarrow$ set of leaf vertices in $G$ with degree 1\;


\For{\rm{\textbf{each}} vertex $v \in IV \cup LV$}{
$c' \leftarrow N(v) \cup \{v\}$\;
\If{$w(c') > \min\{\cup_{c \in C}{score(c,C)}$\}
}{$C \leftarrow C \cup \{c'\}$\;
$c_{min} \leftarrow \arg\min_{c \in C}{score(c, C)}$\;
$C \leftarrow C \backslash c_{min}$\;}
}
\textbf{return} $c$\;
\end{algorithm}
\fi


%\subsection{Find Genes in Local Search}




\subsection{Tabu Search in the Genetic Algorithm}
%Solution-based tabu search methods are widely used in heuristics (mainly local search) for various combinatorial optimization problems, such as the inventory routing problem~\cite{SuTabu} and $p$-next center problem~\cite{ZSL+22}, which prevent the algorithms from duplicated searching for the same solution.
Solution-based tabu search methods are widely used in heuristics (mainly local search) for various combinatorial optimization problems, such as the inventory routing problem~\cite{SuTabu} and $p$-next center problem~\cite{ZSL+22}. In DiverTEAM, we apply solution-based tabu search to the genetic algorithm to prevent the algorithms from searching for the solutions that have been previously encountered and ensure the diversity of the population. 


%During the genetic algorithm procedure, to effectively prevent population convergence, our goal is to eliminate individuals from the population that have been previously encountered. We employ a solution-based tabu approach to ensure genetic diversity. 
Specifically, we establish three hash vectors $H_1, H_2, H_3$ to represent the tabu list. Each vector has a length of $L=10^8$. The three hash vectors are initialized to 0. Additionally, we define three hash functions, denoted as $h_1(\cdot), h_2(\cdot), h_3(\cdot)$, each maps a solution $C$ within the range $[0, L)$. A solution $C$ is considered in the tabu list if $\wedge_{i=1}^{3}H_i(h_i(C)) = 1$. We associate three random integers $j_1(v), j_2(v), j_3(v)$ with each vertex $v$, the hash value $h_i(C), i = (1,2,3)$ can be calculated by $h_i(C) = \sum_{c\in C}\sum_{v\in c} j_i(v) \mod L$.


In the genetic algorithm, each solution $C$ that occurred in the population will be added to the tabu list by setting $\wedge_{i=1}^{3}H_i(h_i(C)) = 1$. And any solution $C$ prohibited by the tabu list will not occur in future populations.


%Additionally, we define a hash function, denoted as $h(S)$, which maps each solution within the range $(0, L]$. If $T(h(S))$ equals $1$, it signifies that the solution is considered tabu.
%To minimize the occurrence of false tabu events, we introduce three separate tabu tables along with their respective hash functions. A solution is deemed tabu only when it is simultaneously marked as tabu in all three tables, i.e, $\wedge_{t=1}^{3}T^t(h^t(S))=1 $. By employing multiple tables and hash functions, we enhance the accuracy of identifying tabu solutions.
%The hash function is defined as equation~\ref{eq_tabu}.

%\begin{equation}
%\label{eq_tabu}
%h^t(C) = \sum_{c\in C}\sum_{v\in c} j^t(v) \mod L
%\end{equation}
%where $j^t(v)$ is a random number for each vertex $v$ within the range $(0, L]$.


\begin{algorithm}[t]
\fontsize{10.1pt}{15}
\caption{PostProcessing($G,C$)}
\label{alg_postprocessing}
\LinesNumbered 
\KwIn{A graph $G=(V,E)$, a solution $C$}
\KwOut{A solution $C$}
%$c \leftarrow$ a random clique in $C$, $C \leftarrow C \backslash \{c\}$\;
%$c \leftarrow$ first clique in $C$\;
$C^* \leftarrow \emptyset$\;
%\For{$i \leftarrow 2:|C|$}{
%\While{$C \neq \emptyset$}{
\For{\rm{\textbf{each}} clique $c\in C$ }{
    %$c \leftarrow$ a random clique in $C$, $C \leftarrow C \backslash \{c\}$\;
    $c \leftarrow c \backslash cov(C^*)$\;
    %\For{\rm{\textbf{each}} vertex $v\in c'$ and $v$ appears in $C^*$}{
    %    $c' \leftarrow c'\backslash\{v\}$\;
    %}
    expand $c$ to maximal, prioritizing vertices that are not in $cov(C^*)$\;
    $C^* \leftarrow C^*\cup \{c\}$\;
}
\For{\rm{\textbf{each}} vertex $v \in V \backslash cov(C^*)$}{
\For{\rm{\textbf{each}} clique $c\in C^*$ }{
%$c' \leftarrow c$, $c' \leftarrow \{v\}$\;
$c' \leftarrow c \backslash \left(V \backslash N(v)\right) \cup \{v\} $\;
%\For{\rm{\textbf{each}} vertex $u \in c$}{
%If{$(u,v) \in E$}{
%    $c' \leftarrow c' \cup \{u\}$\;
%}
%}
\If{$w(C^*\backslash\{c\}\cup \{c'\}) > w(C^*)$}{
    $C^*\leftarrow C^*\backslash\{c\}\cup\{c'\}$,
    \textbf{break}\;
}
}
}
\textbf{return} $C^*$\;
\end{algorithm}

\subsection{Postprocessing}
%Due to the inherent difficulty of obtaining high-quality genes through local search techniques, and the additional challenges associated with applying local search after the genetic algorithm, we employ post-processing methods to identify genetic variants that are better suited for the solution.

We propose two postprocessing methods aiming to further improve each solution $C$ in the population after the genetic algorithm, as depicted in Algorithm~\ref{alg_postprocessing}. The first is a construction heuristic (lines 1-5), which starts from an empty set and iteratively constructs a maximal clique based on parts of each clique $c$ in the input solution $C$. For each clique $c \in C$, the algorithm first removes vertices covered by the current constructed solution $C^*$ from $c$, and then expands it to maximal, preferring vertices not covered by $C^*$. The second is a searching heuristic (lines 6-10), which actually tries to add uncovered vertices to the solution %to improve it.
for possible improvement. 


Note that neither of these two postprocessing methods makes the solution worse. However, they may degrade the quality of the genes and are time-consuming. Thus, we do not use them frequently during the local search or genetic algorithms. When using the postprocessing methods for each individual, we prioritize individuals with larger objective values.


%It is important to note that, for efficiency purposes, post-processing is exclusively performed on solutions of high quality. High-quality solutions are defined as those that achieve results within 0.999 times the current optimal solution.

%For every solution, we employ two post-processing methods as depicted in Algorithm~\ref{alg_postprocessing}. Firstly, we utilize the initial gene in the solution as a foundation. Then, for the remaining genes in the solution, we eliminate the points that already exist within the solution. Afterwards, We prioritize the inclusion of vertices not yet present in the solution, expanding it to its maximal form. Subsequently, for each point that is absent from the solution, we attempt to improve each gene with it. If the transformation results in an improvement, we retain it in the solution. Note that neither of these post-processing methods makes the solution worse.

\subsection{Implementation Details}
\label{sec-Details}
Suppose the cut-off time of the entire algorithm is $t_{max}$. In our implementation, we reserve 6 seconds for postprocessing to try to improve the most promising individuals. Thus the genetic algorithm stops when the running time reaches $t_{max} - 6$ (\ie, stopping condition \textit{\uppercase\expandafter{\romannumeral2}}). And the local search process stops when the running time reaches $t_{max} - 16 - |P| \times k/10$ (\ie, stopping condition \textit{\uppercase\expandafter{\romannumeral1}}). In other words, we reverse $10 + |P| \times k/10$ seconds for the genetic algorithm, where $|P|$ is the population size. These conditions are set empirically. Moreover, in our implementation, the FindGene() function first samples a starting vertex as the initial clique and then extends it as HEA-D~\cite{wu2022head} does. 


Note that DiverTEAM does not restrict the population size but allows it to adjust adaptively according to different instances, making the algorithm more robust and effective.

==> body/abstract.tex <==
In many real-world problems and applications, finding only a single element, even though the best, among all possible candidates, cannot fully meet the requirements. We may wish to have a collection where each individual is not only outstanding but also distinctive. Diversified Top-k (DTk) problems are a kind of combinatorial optimization problem for finding such a promising collection of multiple sub-structures, such as subgraphs like cliques and social communities. In this paper, we address two representative and practical DTk problems, DTk Clique search (DTkC) and DTk Weight Clique search (DTkWC), and propose an efficient algorithm called Diversified Top-k Evolutionary AlgorithM (DiverTEAM) for these two problems. DiverTEAM consists of a local search algorithm, which focuses on generating high-quality and diverse individuals and sub-structures, and a genetic algorithm that makes individuals work as a team and converge to (near-)optima efficiently. Extensive experiments show that DiverTEAM exhibits an excellent and robust performance across various benchmarks of DTkC and DTkWC.
